Your Mega-Constellations Can Be Slim:A Cost-Effective Approach for Constructing Survivable and Performant LEO Satellite Networks

In this paper, we investigate an important research problem facing the upcoming satellite Internet: from a network perspective, how many satellites exactly do we need to construct a survivable and performant LSN? To answer this question, we first formulate the survivable and performant LSN design (SPLD) problem, which aims to find the minimum number of needed satellites to construct an LSN that can provide sufficient amount of redundant paths, required link capacity and acceptable latency for traffic carried by the LSN. Second, to efficiently solve the tricky SPLD problem, we propose MEGAREDUCE, a requirement-driven constellation optimization mechanism, which can calculate feasible solutions for SPLD in polynomial time. Finally, we conduct extensive trace-driven simulations to verify MEGAREDUCE's cost-effectiveness in constructing survivable and performant LSNs on demand, and showcase how MEGAREDUCE can help optimize the incremental deployment and long-term maintenance of future satellite Internet.

==> content/acknowledgement.tex <==
\section{Acknowledgement}
\label{sec:acknowledgement}

We thank all anonymous reviewers for their feedback. This work was supported by the National Key R\&D Program of China (No. 2022YFB3105202), National Natural Science Foundation of China~(NSFC No. 62372259 and No. 62132004). Hewu Li is the corresponding author.
